LO-Det: Lightweight Oriented Object Detection in Remote Sensing Images

A few lightweight convolutional neural network (CNN) models have been recently designed for remote sensing object detection (RSOD). However, most of them simply replace vanilla convolutions with stacked separable convolutions, which may not be efficient due to a lot of precision losses and may not be able to detect oriented bounding boxes (OBB). Also, the existing OBB detection methods are difficult to constrain the shape of objects predicted by CNNs accurately. In this paper, we propose an effective lightweight oriented object detector (LO-Det). Specifically, a channel separation-aggregation (CSA) structure is designed to simplify the complexity of stacked separable convolutions, and a dynamic receptive field (DRF) mechanism is developed to maintain high accuracy by customizing the convolution kernel and its perception range dynamically when reducing the network complexity. The CSA-DRF component optimizes efficiency while maintaining high accuracy. Then, a diagonal support constraint head (DSC-Head) component is designed to detect OBBs and constrain their shapes more accurately and stably. Extensive experiments on public datasets demonstrate that the proposed LO-Det can run very fast even on embedded devices with the competitive accuracy of detecting oriented objects.

==> Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/ZhanchaoHuang.pdf}}]{Zhanchao Huang}
	received the B.E. degree and M.S. degree from Beijing University of Chemical
	Technology, Beijing, China, in 2016 and 2019, respectively. He is currently pursuing the Ph.D. degree with the School of Information and Electronics, Beijing Institute of Technology, Beijing, China. His research interests include object detection and its applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio_photos/WeiLi.pdf}}]{Wei Li}
	(S'11, M'13, SM'16)
	received the B.E.\ degree in telecommunications engineering from Xidian University, Xi'an, China, in 2007, the M.S.\ degree in information science and technology from Sun Yat-Sen University, Guangzhou, China, in 2009, and the Ph.D.\ degree in electrical and computer engineering from Mississippi State University, Starkville, MS, USA, in 2012.
	Subsequently, he spent 1 year as a Postdoctoral Researcher at the University of California, Davis, CA, USA. 
	
	He was a Professor with the College of Information Science
	and Technology at Beijing University of Chemical Technology from 2013 to 2019. He is currently a professor with the School of Information and Electronics, Beijing Institute of Technology. His research interests include hyperspectral image analysis, pattern recognition, and data compression.
		
	He is currently serving as an Associate Editor for the IEEE Signal Processing Letters and the IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing (JSTARS). He has served as Guest Editor for special issue of Journal of Real-Time Image Processing, Remote Sensing, and IEEE JSTARS. He received the 2015 Best Reviewer award from IEEE Geoscience and Remote Sensing Society (GRSS) for his service for IEEE JSTARS and the Outstanding Paper award at IEEE International Workshop on Hyperspectral Image and Signal Processing: Evolution in Remote Sensing (Whispers), 2019.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio_photos/XiangGenXia.pdf}}]{Xiang-Gen Xia}
	(M'97, S'00, F'09) received his B.S. degree in mathematics from Nanjing Normal University, Nanjing, China, and his M.S. degree in mathematics from Nankai University, Tianjin, China, and his Ph.D. degree in electrical engineering  from the University of Southern California, Los Angeles, in 1983, 1986, and 1992, respectively.

	He was a Senior/Research Staff Member at Hughes Research Laboratories, Malibu, California, during 1995-1996. In September 1996, he joined the Department of Electrical and Computer Engineering, University of Delaware, Newark, Delaware, where he is the Charles Black Evans Professor.  
	His current research interests include space-time coding, MIMO and OFDM systems, digital signal processing, and SAR and ISAR imaging. Dr. Xia is the author of the book  Modulated Coding for Intersymbol Interference Channels (New York, Marcel Dekker, 2000).

	Dr. Xia received the National Science Foundation (NSF) Faculty Early Career Development (CAREER) Program Award in 1997, the Office of Naval Research (ONR) Young Investigator Award in 1998, and the Outstanding Overseas Young Investigator Award from the National Nature Science Foundation of China in 2001. He received the 2019 Information Theory Outstanding Overseas Chinese Scientist Award, The Information Theory Society of Chinese Institute of Electronics. Dr. Xia has served as an Associate Editor for numerous international journals including IEEE Transactions on Signal Processing,  IEEE Transactions on Wireless Communications,  IEEE Transactions on Mobile Computing, and   IEEE Transactions on Vehicular Technology. Dr. Xia is Technical Program Chair of the Signal Processing Symp., Globecom 2007 in Washington D.C. and the General Co-Chair of ICASSP 2005 in Philadelphia.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/HaoWang.pdf}}]{Hao Wang}
	received the B.E. degree from Beijing Institute of Technology. Beijing, China, in 2020. He is currently pursuing the M.S. degree with the School of Information and Electronics Beijing Institute of Technology, Beijing, China. His research interest includes object detection and its applications
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_photos/FeiranJie.pdf}}]{Feiran Jie}
 	is a senior engineer of Science and Technology on Electro-Optic Control Laboratory, Luoyang, China. His research interests include image processing and machine vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio_photos/RanTao.pdf}}]{Ran Tao}
	 (Senior Member, IEEE) received the B.S.
	degree from the Electronic Engineering Institute of
	PLA, Hefei, China, in 1985, and the M.S. and Ph.D.
	degrees from the Harbin Institute of Technology,
	Harbin, China, in 1990 and 1993, respectively.

	He was a Senior Visiting Scholar with the University of Michigan, Ann Arbor, MI, USA, and the University of Delaware, Newark, DE, USA, in 2001 and
	2016, respectively. He is a Professor with the School
	of Information and Electronics, Beijing Institute of
	Technology, Beijing, China. He has authored or
	coauthored 3 books and more than 100 peer-reviewed journal articles. His
	research interests include fractional Fourier transform and its applications,
	theory, and technology for radar and communication systems. 
	
	Dr. Tao is a member of the Wireless Communication and Signal Processing
	Commission, URSI. He is a fellow of the Institute of Engineering and
	Technology and the Chinese Institute of Electronics. He was a recipient of
	the National Science Foundation of China for Distinguished Young Scholars
	in 2006, the First Prize of Science and Technology Progress in 2006 and
	2007 awarded by the Ministry of Education, the Distinguished Professor of
	Changjiang Scholars Program in 2009, and the First Prize of Natural Science
	in 2013 awarded by the Ministry of Education. He was a Chief-Professor
	of the Program for Changjiang Scholars and Innovative Research Team in
	University from 2010 to 2012 and has been a Chief-Professor of the Creative
	Research Groups with the National Natural Science Foundation of China since
	2014. He is the Vice-Chair of the IEEE China Council and the International
	Union of Radio Science (URSI) China Council.
\end{IEEEbiography}
